Fine-Tuning Language Models with Just Forward Passes

Fine-tuning language models (LMs) has yielded success on diverse downstream tasks, but as LMs grow in size, backpropagation requires a prohibitively large amount of memory. Zeroth-order (ZO) methods can in principle estimate gradients using only two forward passes but are theorized to be catastrophically slow for optimizing large models. In this work, we propose a memory-efficient zerothorder optimizer (MeZO), adapting the classical ZO-SGD method to operate in-place, thereby fine-tuning LMs with the same memory footprint as inference. For example, with a single A100 80GB GPU, MeZO can train a 30-billion parameter model, whereas fine-tuning with backpropagation can train only a 2.7B LM with the same budget. We conduct comprehensive experiments across model types (masked and autoregressive LMs), model scales (up to 66B), and downstream tasks (classification, multiple-choice, and generation). Our results demonstrate that (1) MeZO significantly outperforms in-context learning and linear probing; (2) MeZO achieves comparable performance to fine-tuning with backpropagation across multiple tasks, with up to 12x memory reduction and up to 2x GPU-hour reduction in our implementation; (3) MeZO is compatible with both full-parameter and parameter-efficient tuning techniques such as LoRA and prefix tuning; (4) MeZO can effectively optimize non-differentiable objectives (e.g., maximizing accuracy or F1). We support our empirical findings with theoretical insights, highlighting how adequate pre-training and task prompts enable MeZO to fine-tune huge models, despite classical ZO analyses suggesting otherwise.

==> descent_lemma.tex <==

\section{Descent Lemma}
Define the gradient estimate $\hat\nabla L(x)$:
\begin{align}
	\hat\nabla L(x) = \E_{i\in B, j\in[n]} \left[\frac{L_i(x+\eps z_j) - L_i(x-\eps z_j)}{2\eps} dz_j\right]  
	\approx d\E_{ij} (\nabla L_i\cdot z_j)z_j
\end{align}
where $L_i$ is the loss on the $i$th datapoint out of a batch of $B$ datapoints and $n$ noise vectors are sampled.
We can write a term in the covariance:
$$ d^2\E_{i_1,i_2,j_1,j_2} [\nabla L_{i_1}z_{j_1}z_{j_1}z_{j_2}z_{j_2}\nabla L_{i_2}] $$
Now, we can write
\begin{align*}
\frac 1n \left[(\nabla L_{i_1} \nabla L_{i_2}) I + 2\nabla L_{i_1}\nabla L_{i_2}^\top \right] + \frac{n-1}{n} \nabla L_{i_1}\nabla L_{i_2}^\top = \frac 1n \left[(\|\nabla L\|^2 + \frac 1B \tr(\Sigma_B))I\right] + \frac{n+1}{n}\left[\nabla L \nabla L^\top + \frac 1B \Sigma_B\right]
\end{align*}
So when we expand the update we get
$$ -\frac\eta 2 \|\nabla L\|^2 + \frac{\eta^2}{2} \langle \Sigma, H\rangle = -\frac\eta 2 \|\nabla L\|^2 + \frac{\eta^2}{2n}\tr(H)\left(\|\nabla L\|^2 + \frac 1B \tr(\Sigma_B)\right) + \frac{\eta^2}{2}\frac{\langle \Sigma_B, H\rangle}{B} $$
From this, we get four conditions on $\eta$:
\begin{enumerate}
	\item $\eta\leq 1/\|H\|_2$
	\item $\eta\leq n/\tr(H)$	
	\item $$\eta\leq \frac{nB\|\nabla L\|^2}{\tr(H)\tr(\Sigma)}$$
	\item $$\eta\leq \frac{B\|\nabla L\|^2}{\langle H, \Sigma\rangle}$$
\end{enumerate}
The second condition is not important since $B$ is small. 
So we have to compare conditions 3 and 4. 
If we follow the least squares loss logic, we can handwave $\Sigma\sim L\cdot H$. 
Then, it becomes $n$ vs $r$ where $r = \tr H / \|H\|_2$ (I think?)


==> dimension_free_rate.tex <==
\section{Dimension Free Rate}

For now we prove the dimension free rate in the kernel setting where $\ell(\hat y, y) = \frac12(\hat y - y)^2$ is the square loss. \enote{how to extend to more general loss functions?}

In the kernel regime, we have
\begin{align*}
    L(\theta) &= \frac{1}{N}\sum_{i=1}^N \frac12(f(\theta, x_i) - y_i)^2\\
    \nabla L(\theta) &= \frac{1}{N}\sum_{i=1}^N (f(\theta, x_i) - y_i)\phi(x_i)\\
    \nabla^2 L(\theta) &= \frac{1}{N}\sum_{i=1}^N \phi(x_i)\phi(x_i)^T.
\end{align*}
Since the Hessian is constant, we denote it by $\nabla^2 L$. We see that $\nabla^2L$ is rank at most $N$, and thus $\tr(\nabla^2L) \le N\ell$.

In general, the minibatch covariance $\Sigma_{MB}$ is given by
\begin{align*}
    \Sigma_{MB}(\theta) = \frac{1}{N}\sum_{i=1}^N \ell'(f(\theta, x_i), y_i)^2\phi(x_i)\phi(x_i)^T - \nabla L(\theta)\nabla L(\theta)^T.
\end{align*}

In the case of square loss, this is
\begin{align*}
    \Sigma_{MB}(\theta) = \frac{1}{N}\sum_{i=1}^N (f(\theta, x_i) - y_i)^2\phi(x_i)\phi(x_i)^T - \nabla L(\theta)\nabla L(\theta)^T
\end{align*}
\anote{Why is this necessary here? All these scalings change with different loss functions $\ell(f,y)$}
We handwave slightly and say all the residuals are of the same scale, in which case we have $\Sigma_{MB}(\theta) \approx L(\theta)\cdot \nabla^2L - \nabla L(\theta)\nabla L(\theta)^T$. We can also make the upper bound
\begin{align*}
    \Sigma_{MB}(\theta) \preceq \max_{i \in [N]} (f(\theta, x_i) - y_i)^2 \cdot \frac{1}{N}\sum_{i=1}^N \phi(x_i)\phi(x_i)^T \preceq N L(\theta) \cdot \nabla^2L
\end{align*}

\enote{can we make the handwavy thing rigorous and save a factor of $N$?}
\snote{If you use the ``natural task in the infinite-width limit'' assumption from the other kernel paper, you can say that $(f(\theta, x_i) - y_i)$ decays with the width...but it will kind of change the flavor of the theorem statement. This will also allow you to choose arbitrary loss functions...}

For a general loss function, our gradient estimate satisfies (here $z_j \sim \mathcal{N}(0, I_d)$)
\begin{align*}
    \hat \nabla L(\theta) &= \mathbb{E}_{i, j}\left[\frac{L_i(x + \epsilon z_j) - L_i(x - \epsilon z_j)}{2\epsilon}z_j\right]\\
    &= \mathbb{E}_{i,j}[z_jz_j^T\nabla L_i] + O(\mathbb{E}_{j}[\rho\epsilon^2\norm{z_j}^43])\\
    &= \mathbb{E}_{i,j}[z_jz_j^T\nabla L_i] + O(\rho\epsilon^2d^2)
\end{align*}
where we assume $L$ is $\rho$-Hessian Lipschitz. In the case of kernel regime/square loss, $\rho = 0$, and $\hat \nabla L(\theta) = \mathbb{E}_{i,j}[z_jz_j^T\nabla L_i]$; this is also now an unbiased estimator of the gradient.

\snote{What's $n$ below?}\anote{$n$ is number of $z$s sampled} Given a gradient estimate $\hat \nabla L(\theta)$, the descent lemma gives
\begin{align*}
    &\mathbb{E}[L(\theta_{t+1}) \mid \theta_t]\\
    &= L(\theta_t) - \eta\norm{\nabla L(\theta_t)}^2 + \frac12\eta^2\langle \nabla^2L, \mathbb{E}[\hat \nabla L(\theta)\hat \nabla L(\theta)^T] \rangle\\
    &= L(\theta_t) - \eta\norm{\nabla L(\theta_t)}^2 + \frac{\eta^2}{2n}\left(\norm{\nabla L}^2 + \frac{1}{B}\tr(\Sigma_{MB})\right)\tr(\nabla^2 L) + \frac{\eta^2(n+1)}{2n}\left(\nabla L(\theta_t)^T\nabla^2L \nabla L(\theta_t) + \frac{1}{B}\langle \Sigma_{MB}, \nabla^2L\rangle\right)
\end{align*}

Let $\eta \le \min \left(\frac{1}{4\ell}, \frac{n}{2N\ell}, \right)$. Then
\begin{align*}
    \frac{\eta^2(n+1)}{2n}\nabla L(\theta_t)^T\nabla^2L \nabla L(\theta_t) &\le \eta^2\ell\norm{L(\theta_t)}^2\cdot \le \frac{\eta}{4}\norm{\nabla L(\theta_t)}^2\\
    \frac{\eta^2}{2n}\norm{\nabla L(\theta_t)}^2\tr(\nabla^2L) &\le  \frac{\eta^2N\ell}{2n}\norm{\nabla L(\theta_t)}^2 \le \frac{\eta}{4}\norm{\nabla L(\theta_t)}^2.
\end{align*}
Then
\begin{align*}
    \mathbb{E}[L(\theta_{t+1}) \mid \theta_t] - L(\theta_t) &\le -\frac{\eta}{2}\norm{\nabla L(\theta_t)}^2 + \frac{\eta^2}{2nB}\tr(\Sigma_{MB})\tr(\nabla^2L) + \frac{\eta^2(n+1)}{2nB}\langle \Sigma_{MB}, \nabla^2L\rangle\\
    &\le -\frac{\eta}{2}\norm{\nabla L(\theta_t)}^2 + \frac{\eta^2}{2nB}NL(\theta_t)\tr(\nabla^2L)^2 + \frac{\eta^2(n+1)}{2nB}NL(\theta)\norm{\nabla^2L}_F^2\\
    &\le -\frac{\eta}{2}\norm{\nabla L(\theta_t)}^2 + \frac{\eta^2\ell^2}{2nB}N^3L(\theta_t) + \frac{\eta^2(n+1)}{2nB}N^2\ell^2L(\theta)\\
    &= -\frac{\eta}{2}\norm{\nabla L(\theta_t)}^2 + \frac{\eta^2\ell^2N^2}{B}(\frac{N}{2n} + 1)L(\theta_t)\\
\end{align*}
Additionally,
\begin{align*}
    \norm{\nabla L(\theta_t)}^2 \ge 2L(\theta_t)\lambda_N(\nabla^2L).
\end{align*}
Thus
\begin{align*}
    \mathbb{E}[L(\theta_{t+1}) \mid \theta_t] \le L(\theta_t)\left(1 + \frac{\eta^2\ell^2N^2}{B}(\frac{N}{2n} + 1) - \eta \lambda_N(\nabla^2L)\right)
\end{align*}
For $\eta \le \frac{\lambda_N B}{2\ell^2N^2(\frac{N}{2n} + 1)}$, we get
\begin{align*}
    \mathbb{E}[L(\theta_{t+1}) \mid \theta_t] \le (1 - \eta \lambda_N)L(\theta_t).
\end{align*}
The iteration complexity to reach $\epsilon$ loss is thus
\begin{align*}
    \frac{1}{\eta\lambda_N}\log\frac{1}{\epsilon}.
\end{align*}
Selecting $\eta = \min \left(\frac{1}{4\ell}, \frac{n}{2N\ell}, \frac{\lambda_N B}{2\ell^2N^2(\frac{N}{2n} + 1)} \right)$ yields an iteration complexity of 
\begin{align*}
    \tilde O\left( \frac{\ell}{\lambda_N} +  \frac{\ell}{\lambda_N}\cdot \frac{N}{n} + \frac{\ell^2}{\lambda_N^2}N^2(\frac{N}{2n} + 1)\cdot\frac{1}{B}\right) = \tilde O \left((\kappa + \frac{\kappa^2N^2}{B})(1+ \frac{N}{n}\right),
\end{align*}
where $\kappa = \ell/\lambda_N$. Crucially, this rate is dimension independent.

\enote{does minibatch SGD rate not have this $\kappa^2N^2$ term? Usually its written in terms of $\sigma^2 := \tr(\Sigma_B)$, but in this derivation I did $\tr(\Sigma_B) \lesssim N\tr(\nabla^2L) \le N^2\ell$ which is where this term comes from}.

\anote{This seems somewhat loose. I think it's worth separating the fast rates for minibatch SGD with square loss from the ZO stuff, can plug in later if needed.}


\section{Rate comparison}

\enote{for now working in kernel regime + square loss setting. TODO can we extend this to something more general.}

In the worst case, zeroth-order optimization algorithms can have rates which are a dimension factor worse than their first-order counterparts. We show, however, that when the Hessian has a low-rank structure, that the slowdown due to zeroth-order optimization only scales with the effective rank of the Hessian. In the case of fine-tuning large language models, the effective Hessian rank is much smaller than the parameter count.

We first quantify the loss decrease prescribed by the descent lemma in the case of minibatch SGD (i.e with gradient queries). In minibatch SGD with a batch size of $B$, the gradient estimate is $\hat L(\theta) = \E_{i \sim [B]}[\nabla L_i]$, and thus the covariance is
\begin{align*}
    \mathbb{E}[\hat \nabla L(\theta)\hat \nabla L(\theta)^T] = \frac{1}{B}\Sigma_{MB}(\theta) + \nabla L(\theta)\nabla L(\theta)^T.
\end{align*}
The descent lemma for minibatch SGD is thus
\begin{align*}
    \E[L(\theta_{t+1}) \mid \theta_t] - L(\theta_t) &=  - \bar\eta\norm{\nabla L(\theta_t)}^2 + \frac12 \bar\eta^2\langle \nabla^2L, \mathbb{E}[\hat \nabla L(\theta)\hat \nabla L(\theta)^T] \rangle\\
    &\le - (\bar\eta - \frac12\bar\eta^2\ell)\norm{\nabla L(\theta_t)}^2 + \frac{\bar\eta^2}{2B} \langle \Sigma_{MB}(\theta_t), \nabla^2L \rangle.
\end{align*}
Choosing a learning rate of $\bar\eta \le \frac{1}{\ell}$ yields
\begin{align*}
    \E[L(\theta_{t+1}) \mid \theta_t] \le L(\theta_t) - \frac{\bar\eta}{2}\norm{\nabla L(\theta_t)}^2 + \frac{\bar\eta^2 \ell}{2B}\tr(\Sigma_{MB}(\theta_t)).
\end{align*}

We next define the notion of effective rank:
\begin{definition}
Let $r = \tr(\nabla^2L)/\norm{\nabla^2 L}_{op}$ denote the \emph{effective rank} of the Hessian.
\end{definition}

The following theorem shows that a single step of ZO-SGD decreases the loss by at least a $\frac{n}{n + r + 1}$ fraction of the loss decrease prescribed by the descent lemma for minibatch SGD:

\begin{theorem}
Let $\eta = \frac{n}{n + r + 1}\cdot \bar \eta$, where $\bar\eta \le \frac{1}{\ell}$. Then if $\theta_{t+1} = \theta_t - \eta \hat \nabla L(\theta_t)$ is a single step of ZO-SGD starting at $\theta_t$ with learning rate $\eta$, we can bound the loss decrease by
\begin{align*}
    \E[L(\theta_{t+1}) \mid \theta_t] - L(\theta_t) \le \frac{n}{n + r + 1}\cdot\left[-\frac{\bar \eta}{2}\norm{\nabla L(\theta_t)}^2 + \frac{\bar \eta^2 \ell}{2B}\tr(\Sigma_{MB}(\theta_t)) \right]
\end{align*}
\end{theorem}

\begin{proof} 
By Taylor's theorem with remainder, we have that
\begin{align*}
    \cL(\btheta_{t+1}) = \cL(\btheta_t) + \nabla \cL(\btheta_t)^T(\btheta_{t+1} - \btheta_t) + \int_0^1 \lambda (\btheta_{t+1} - \btheta_t)^T\nabla^2 \cL(\lambda\btheta_{t+1} + (1-\lambda)\btheta_t)(\btheta_{t+1} - \btheta_t)^Td\lambda
\end{align*}
Next, we use the assumption that $\nabla^2 \cL(\lambda\btheta_{t+1} + (1-\lambda)\btheta_t) \preceq \bH(\btheta_t)$ to get
\begin{align*}
    \cL(\btheta_{t+1}) &\le \cL(\btheta_t) + \nabla \cL(\btheta_t)^T(\btheta_{t+1} - \btheta_t) +(\btheta_{t+1} - \btheta_t)^T\bH(\btheta_t)(\btheta_{t+1} - \btheta_t)\\
    & = \cL(\btheta_t) - \eta\nabla \cL(\btheta_t)^T \hat \nabla \cL(\btheta_t; \cB) + \frac12\eta^2\hat \nabla \cL(\btheta_t; \cB)^T\bH(\btheta_t)\hat \nabla \cL(\btheta_t; \cB).\\
\end{align*}
Taking the conditional expectation with respect to $\btheta_t$ and plugging in the formula for the covariance of our ZO estimate $\hat \nabla \cL(\btheta_t; \cB)$ yields
\begin{align*}
    \E[\cL(\btheta_{t+1}) \mid \btheta_t] &\le \cL(\btheta_t) - \eta\norm{\nabla \cL(\btheta_t)}^2 + \frac{\eta^2}{2}\left\langle \bH(\btheta_t), \E\left[\hat \nabla \cL(\btheta; \mathcal{B})\hat \nabla \cL(\btheta; \mathcal{B})^T\right] \right\rangle\\
    &= \cL(\btheta_t) - \eta\norm{\nabla \cL(\btheta_t)}^2 + \frac{\eta^2}{2k}\left(\norm{\nabla \cL(\btheta_t)}^2 + \frac{1}{B}\tr(\bSigma_{MB}(\btheta_t))\right)\tr(\bH(\btheta_t))\\
    &\qquad + \frac{\eta^2(k+1)}{2k}\left(\nabla \cL(\btheta_t)^T\bH(\btheta_t) \nabla \cL(\btheta_t) + \frac{1}{B}\langle \bSigma_{MB}(\btheta_t), \bH(\btheta_t)\rangle\right)\\
    &= \cL(\btheta_t) - \left(\eta - \frac{\eta^2}{2k}\tr(\bH(\btheta_t)) - \frac{\eta^2\ell(k+1)}{2k}\right)\norm{\nabla \cL(\btheta_t; \cB)}^2 + \frac{\eta^2}{2kB}\tr(\bSigma_{MB}(\btheta_t))\tr(\bH(\btheta_t))\\
    &\qquad + \frac{\eta^2(k+1)}{2kB}\langle \bSigma_{MB}(\btheta_t), \bH(\btheta_t) \rangle.
\end{align*}
% The descent lemma for our gradient estimate $\hat \cL(\btheta_t; \cB)$ yields \enote{move derivation for covariance estimate from other section here}
% Since the loss is $\ell$-smooth, we have
% \begin{align*}
%     E[L(\theta_{t+1} \mid \theta_t) \le L(\theta_t) - \eta\norm{\nabla L(\theta_t)}^2 + \frac{\eta^2\ell}{2}\E[\norm{\hat \nabla L(\theta_t)}^2]
% \end{align*}
% \begin{align*}
%     &\E[L(\theta_{t+1}) \mid \theta_t]\\
%     &= L(\theta_t) - \eta\norm{\nabla L(\theta_t)}^2 + \frac{\eta^2}{2n}\left(\norm{\nabla L}^2 + \frac{1}{B}\tr(\Sigma_{MB})\right)\tr(\nabla^2 L) + \frac{\eta^2(n+1)}{2n}\left(\nabla L(\theta_t)^T\nabla^2L \nabla L(\theta_t) + \frac{1}{B}\langle \Sigma_{MB}, \nabla^2L\rangle\right)\\
%     &\le L(\theta_t) - \left(\eta - \frac{\eta^2}{2n}\tr(\nabla^2L) - \frac{\eta^2\ell(n+1)}{2n}\right)\norm{\nabla L(\theta_t)}^2 + \frac{\eta^2}{2nB}\tr(\Sigma_{MB}(\theta_t))\tr(\nabla^2 L) + \frac{\eta^2(n+1)}{2nB}\langle \Sigma_{MB}(\theta_t), \nabla^2L \rangle.
% \end{align*}
By assumption, the Hessian upper bound $\bH(\btheta_t)$ satisfies $\tr(\bH(\theta_t)) \le \ell r$. Furthermore, since $\eta = \frac{n}{n + r + 1}\cdot \bar \eta \le \frac{1}{\ell}\cdot \frac{n}{n + r + 1}$. From this we get that
\begin{align*}
    \frac{\eta^2}{2n}\tr(\bH(\btheta_t)) + \frac{\eta^2\ell(n+1)}{2n} \le \frac{\eta^2}{2n}(\ell r + \ell(n+1)) \le \frac{\eta}{2}
\end{align*}
and thus
\begin{align*}
    \E[\cL(\btheta_{t+1}) \mid \btheta_t] &\le \cL(\btheta_t) - \frac{\eta}{2}\norm{\nabla \cL(\btheta_t; \cB)}^2 + \frac{\eta^2}{2B}\left(\frac{1}{n}\tr(\bSigma_{MB}(\btheta_t))\tr(\bH(\btheta_t)) + \frac{n+1}{n}\langle \bSigma_{MB}(\btheta_t), \bH(\btheta_t)\right)\\
    &\le \cL(\btheta_t) - \frac{\eta}{2}\norm{\nabla \cL(\btheta_t; \cB)}^2 + \frac{\eta^2\ell}{2B}\cdot\frac{n + r + 1}{n}\tr(\bSigma_{MB}(\btheta_t))\\
    &= \cL(\btheta_t) - \frac{n}{n + r + 1}\cdot\left[\frac{\bar \eta}{2}\norm{\nabla \cL(\btheta_t; \cB)}^2 - \frac{\bar \eta^2 \ell}{2B}\tr(\bSigma_{MB}(\btheta_t)) \right],
\end{align*}
as desired.
\end{proof}


==> kernel_analysis.tex <==
\section{Kernel Analysis}
Suppose the predictor $f$ has a kernel form like $f(\theta, x) = \phi(x)\cdot\theta$. 
Then, we can write the loss, gradient, and Hessian:
\begin{align}
	L &= \frac 1N \sum_{i=1}^N \ell(f_i,y_i) = \frac 1N \sum_i \ell(\phi(x_i)\cdot\theta, y_i) \\
	\nabla L &= \frac 1N \sum_i \ell'(\phi(x_i)\cdot\theta, y_i) \cdot \phi(x_i) \\
	\nabla^2 L &= \frac 1N \sum_i \ell''(\phi(x_i)\cdot\theta, y_i) \phi(x_i)\phi(x_i)^\top \\
	\tr(\nabla^2 L) &= \frac 1N \sum_i \ell''(\phi(x_i)\cdot \theta, y_i) \|\phi(x_i)\|^2
\end{align}
The Hessian $H$ for any $f$ can be split as 
\begin{align}
	H &= \sum_i \ell''\nabla f\nabla f^\top + \sum \ell'\nabla^2 f \\
	\tr(H) &= \sum_i \ell''\|\nabla f\|^2 + \sum \ell''\tr(\nabla^2 f) 	
\end{align}
The kernel assumption allows us to model the first term of this Hessian, so we hope that the second term $\sum\ell'\tr(\nabla^2 f)$ is small. 
There is probably some tradeoff then, where large $\eps$ makes the gradient estimate worse but also speeds up optimization.

==> random_stuff.tex <==
\section{Random stuff}
\subsection{Regularization term}
We were wondering why setting $\epsilon$ much larger than $\eta$ even makes sense. 
First, we Taylor expand 
$$ \frac{L(\theta + \eps z) - L(\theta - \eps z)}{2\eps} z$$
Then the third order term is
$$\frac{3\eps^2}{2} \nabla^3 L(z^{\otimes 3}) z$$
Then,
$$ \E[z^4(\nabla^3 L)] = 3I^2 (\nabla^3 L) = 3\nabla^3 L(I) = \nabla \tr(\nabla^2 L)$$
so using the zeroth order estimate implicitly regularizes the trace of the Hessian.

==> tables/generation_results.tex <==

% \captionsetup[wrapfigure]{name=Table}


% \begin{wrapfigure}{r}{0.4\textwidth}
% \begin{minipage}{0.4\textwidth}

\begin{table}[t]
\centering
\small
% \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{lccc}
    \toprule
     Task  & \tf{SQuAD} & \tf{SQuAD v2} & \tf{DROP} \\
    % Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
    \midrule
    % \midrule
    Zero-shot & 46.2 & 21.4\\
    ICL & 75.9 & 44.6 \\
    LP \\
    ZO & \\
    ZO-LoRA & \\
    ZO-Prefix &  \\
    \midrule
    1.3B FT &  \\
    13B FT \\
    \bottomrule
    \end{tabular}
    %}
    \caption{
        Generation tasks
    }
    \label{tab:gen}
\end{table}
% \end{minipage}
% \end{wrapfigure}


% \begin{table*}[t]
%     \centering
%     \small
%         \begin{tabular}{lcccccc}
%         \toprule
%          Task  &  \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{TREC}} \\
%         Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
%         % eNTK solves task & \checkmark & \checkmark & \checkmark & \checkmark & (\checkmark) & \checkmark & & \checkmark & & & (\checkmark) & \checkmark & \checkmark & \checkmark\\
%         % Linearization & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & \checkmark & \checkmark & \checkmark & \checkmark  \\
%         % Fixed Features & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
%         % \midrule
%         % Kernel behavior & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & (\checkmark) & \checkmark & \checkmark & \checkmark \\
%         \midrule
%         Zero-shot & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0 \\
%         \midrule
%         \multicolumn{7}{c}{Gradient-based methods: $16$-shot} \\
%         \midrule
%         Adam FT \\
%         SGD FT \\
%         LP-FT \\
%         LoRA FT \\
%         Prefix FT \\
%         \midrule
%         \multicolumn{7}{c}{Gradient-free methods: $16$-shot} \\
%         \midrule
%         LP \\
%         ZO-SGD \\
%         ZO-Adam \\
%         LP-ZO-SGD \\
%         ZO-LoRA \\
%         ZO-Prefix \\
%         
%         \midrule
%         
%         \bottomrule
%         \end{tabular}
%         \caption{
%         Experiments on RoBERTa-large    
%         }
%         \label{tab:summary}
%     \end{table*}

% \begin{table*}[t]
%     \centering
%     \resizebox{0.98\linewidth}{!}{
%         \begin{tabular}{lcccccc|cccccc}
%         \toprule
%         & \multicolumn{6}{c}{\textbf{$16$ examples per class}} & \multicolumn{6}{c}{\textbf{$512$ examples per class}}\\
%         \cmidrule(lr){2-7}\cmidrule(lr){8-13}
%          Task  &  \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c|}{\textbf{TREC}} & \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{TREC}} \\
%         Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c|}{-- topic clf. --}& \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
%         % eNTK solves task & \checkmark & \checkmark & \checkmark & \checkmark & (\checkmark) & \checkmark & & \checkmark & & & (\checkmark) & \checkmark & \checkmark & \checkmark\\
%         % Linearization & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & \checkmark & \checkmark & \checkmark & \checkmark  \\
%         % Fixed Features & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
%         % \midrule
%         % Kernel behavior & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & (\checkmark) & \checkmark & \checkmark & \checkmark \\
%         %\midrule
%         Zero-shot & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0 & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0\\
%         \midrule
%         \multicolumn{13}{c}{Gradient-based methods} \\
%         \midrule
%         FT \\
%         % SGD FT \\
%         % LP-FT \\
%         LoRA FT \\
%         Prefix FT \\
%         \midrule
%         \multicolumn{13}{c}{Gradient-free methods} \\
%         \midrule
%         LP & 76.0 (2.8)	& 40.3 (1.9) & 66.0 (2.7) & 56.5 (2.5) & 59.4 (5.3)	& 51.3 (5.5)\\
%         ZO \\
%         % ZO-Adam \\
%         % LP-ZO-SGD \\
%         ZO-LoRA \\
%         ZO-Prefix \\
%         
%         \midrule
%         
%         \bottomrule
%         \end{tabular}}
%         \caption{
%         Experiments on RoBERTa-large    
%         }
%         \label{tab:summary}
%     \end{table*}

==> tables/largeandnondiff.tex <==

\begin{table}[h]
% \small
%\resizebox{0.99\textwidth}{!}{
\begin{subtable}[b]{0.46\textwidth}
\centering
    \resizebox{0.99\textwidth}{!}{
        \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lcccccc}
    \toprule
     Task  & \tf{SST-2} & \tf{RTE} & \tf{BoolQ} & \tf{WSC} & \tf{WIC} & \tf{SQuAD} \\
    % Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
    \midrule
    % \midrule
    Zero-shot & 56.7 & 52.0 & 39.1 & 38.5 &	50.2 & 46.5\\
    ICL & 81.9 & 66.8 & 66.2 &56.7&	51.3 & 78.0\\
    \mezo{} &  \tf{90.6} & \tf{72.6} & \tf{73.5} & \tf{63.5} & \tf{59.1} & \tf{85.2}\\
    \midrule
    Zero-shot & 57.5 & 67.2 & 66.8&	43.3& 50.6&48.1\\
    ICL & 89.3 & 65.3&	62.8&	52.9&54.9&81.3\\
    \mezo{} & \tf{93.6} & 66.1$^\dagger$ & \tf{72.7$^\dagger$} & \tf{63.5} &\tf{58.9} & 79.9$^\dagger$ \\
    \bottomrule
    \end{tabular}}%}
   % \vspace{5pt}
    \caption{
        Experiments on OPT-30B and OPT-66B (with 1,000 examples). 
        We report the best of \mezo{} and \mezo{} (prefix). See \Cref{app_sec:opt_more} for more results.
        We see that on most tasks 
        \mezo{} effectively optimizes up to 66B models and outperforms zero-shot and ICL. 
        $\dagger$: use fewer training steps due to compute budget limit, which will be updated in later revision.
        % \tnote{$\dagger$: limited steps (5000)}.
    }
    \label{tab:combo_large}
\end{subtable}
%\hfill
\begin{subtable}[b]{0.51\textwidth}

\centering
    \resizebox{0.99\textwidth}{!}{
        \setlength{\tabcolsep}{3pt}
        \begin{tabular}{lccccc}
            \toprule
             Model & \multicolumn{4}{c}{RoBERTa-large (350M)} & OPT-13B \\
             Task  & \tf{SST-2} & \tf{SST-5} & \tf{SNLI} & \tf{TREC}  & \tf{SQuAD} \\
            % Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
            \midrule
            % \midrule
            Zero-shot & 79.0 & 35.5& 50.2 & 32.0  & 46.2\\
            % Cross Entropy (FT) & 93.9 (0.7) &  88.7 (0.8) & 97.3 (0.2) & 84.9 \\
            % Cross Entropy (ZO) & 93.3 (0.7) & 83.0 (1.0) & 94.3 (1.3) \\
            % Accuracy/F1 & 92.7 (1.1) & 82.7 (1.0) & 68.6 (5.9) \\
            CE (FT) & 93.9 & 55.9 &  88.7  & 97.3  & 84.2 \\
            CE (\mezo{}) & 93.3 & 53.2 & 83.0  & 94.3  & 84.7\\
            ACC/F1 (\mezo{}) & 92.7 &  48.9 & 82.7  & 68.6 & 78.5 \\
            \bottomrule
            \end{tabular}} % }
            %\vspace{5pt}
            \caption{
                \mezo{} with non-differentiable objectives. For classification tasks ($k=512$), we use \mezo{} with full-parameter and accuracy as objective; for SQuAD (1,000 examples), we use \mezo{} (prefix) and F1 as objective. % \danqi{How many examples are used? You only mentioned $k = 512$ for classification tasks.}
                % \snote{TG, add the other SST-5 numbers (table has disappeared lol)}
                % Non-differentiable objective. $k=512$ for RoBERTa-large, 100K steps. For RoBERTa-large we use ZO and for OPT-13B we use ZO-prefix.
            }
            \label{tab:combo_nondiff}
        \end{subtable}

\end{table}

==> tables/more_roberta_large.tex <==


\begin{table*}[h]
% \captionsetup[wrapfigure]{name=Table}

%     \begin{wrapfigure}{r}{0.65\textwidth}
%         \begin{minipage}{0.65\textwidth}
\centering
% \small
\resizebox{0.95\textwidth}{!}{
    \setlength{\tabcolsep}{0.3cm}
    \begin{tabular}{lcccccc}
    \toprule
     Task  &  \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{TREC}} \\
    Task type & \multicolumn{2}{c}{------ sentiment ------} & \multicolumn{3}{c}{------ natural language inference ------} & \multicolumn{1}{c}{--- topic ---}\\
    % eNTK solves task & \checkmark & \checkmark & \checkmark & \checkmark & (\checkmark) & \checkmark & & \checkmark & & & (\checkmark) & \checkmark & \checkmark & \checkmark\\
    % Linearization & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & \checkmark & \checkmark & \checkmark & \checkmark  \\
    % Fixed Features & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
    % \midrule
    % Kernel behavior & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & (\checkmark) & \checkmark & \checkmark & \checkmark \\
    \midrule
        Zero-shot & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0 \\
\midrule

    \multicolumn{7}{c}{Gradient-free methods: $k=16$}\\%16 examples per class} \\
    \midrule
    LP & 76.0 (2.8)	& 40.3 (1.9)	&66.0 (2.7)	&56.5 (2.5)	&59.4 (5.3)	&51.3 (5.5) \\
    ZO & 90.5 (1.2)	& 45.5 (2.0)	&68.5 (3.9)	&58.4 (2.8)$\dagger$ & 64.0 (3.3) &76.9 (2.7) \\
    % ZO \\
    % LP-ZO-SGD \\
    ZO-LoRA & 91.4 (0.9) & 43.0 (1.6) & 69.7 (6.0)&64.0 (2.5) & 64.9 (3.6) &73.1 (6.5)$\dagger$\\
    ZO-prefix & 90.8 (1.7)	&45.8 (2.0)&	71.6 (2.5)	&&&80.3 (3.6) \\
        \midrule
    \multicolumn{7}{c}{Gradient-based methods: $k=16$}\\% 16 examples per class} \\
    \midrule
    FT & 92.1 (1.8)	& 47.8 (1.8) & 75.9 (3.1) \\
    % SGD FT \\
    % LP-FT \\
    FT-LoRA \\
    FT-prefix & 91.9 (1.0)&47.7 (1.1) & 77.2 (1.3) & 66.5 (2.5)	&66.6 (2.0)	&85.7 (1.3) \\
    % \midrule
    % \midrule
    \midrule
    \multicolumn{7}{c}{$k=512$}\\ % examples per class} \\
    \midrule
    LP \\
    ZO \\
    ZO-prefix & 93.3 (0.1)	& 53.6 (0.5)	&84.8 (1.1) &	79.8 (1.2) & & 94.4 (0.7)  \\
    FT \\
    % \midrule
    % \multicolumn{7}{c}{Gradient-free methods: 512 examples per class} \\
    % \midrule

    \bottomrule
    \end{tabular}}
    \caption{
    Experiments on RoBERTa-large    
    }
    \label{tab:roberta_more}
\end{table*}
% \end{minipage}
% \end{wrapfigure}


% \begin{table*}[t]
%     \centering
%     \small
%         \begin{tabular}{lcccccc}
%         \toprule
%          Task  &  \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{TREC}} \\
%         Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
%         % eNTK solves task & \checkmark & \checkmark & \checkmark & \checkmark & (\checkmark) & \checkmark & & \checkmark & & & (\checkmark) & \checkmark & \checkmark & \checkmark\\
%         % Linearization & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & \checkmark & \checkmark & \checkmark & \checkmark  \\
%         % Fixed Features & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
%         % \midrule
%         % Kernel behavior & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & (\checkmark) & \checkmark & \checkmark & \checkmark \\
%         \midrule
%         Zero-shot & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0 \\
%         \midrule
%         \multicolumn{7}{c}{Gradient-based methods: $16$-shot} \\
%         \midrule
%         Adam FT \\
%         SGD FT \\
%         LP-FT \\
%         LoRA FT \\
%         Prefix FT \\
%         \midrule
%         \multicolumn{7}{c}{Gradient-free methods: $16$-shot} \\
%         \midrule
%         LP \\
%         ZO-SGD \\
%         ZO-Adam \\
%         LP-ZO-SGD \\
%         ZO-LoRA \\
%         ZO-Prefix \\
%         
%         \midrule
%         
%         \bottomrule
%         \end{tabular}
%         \caption{
%         Experiments on RoBERTa-large    
%         }
%         \label{tab:summary}
%     \end{table*}

% \begin{table*}[t]
%     \centering
%     \resizebox{0.98\linewidth}{!}{
%         \begin{tabular}{lcccccc|cccccc}
%         \toprule
%         & \multicolumn{6}{c}{\textbf{$16$ examples per class}} & \multicolumn{6}{c}{\textbf{$512$ examples per class}}\\
%         \cmidrule(lr){2-7}\cmidrule(lr){8-13}
%          Task  &  \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c|}{\textbf{TREC}} & \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{TREC}} \\
%         Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c|}{-- topic clf. --}& \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
%         % eNTK solves task & \checkmark & \checkmark & \checkmark & \checkmark & (\checkmark) & \checkmark & & \checkmark & & & (\checkmark) & \checkmark & \checkmark & \checkmark\\
%         % Linearization & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & \checkmark & \checkmark & \checkmark & \checkmark  \\
%         % Fixed Features & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
%         % \midrule
%         % Kernel behavior & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & (\checkmark) & \checkmark & \checkmark & \checkmark \\
%         %\midrule
%         Zero-shot & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0 & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0\\
%         \midrule
%         \multicolumn{13}{c}{Gradient-based methods} \\
%         \midrule
%         FT \\
%         % SGD FT \\
%         % LP-FT \\
%         LoRA FT \\
%         Prefix FT \\
%         \midrule
%         \multicolumn{13}{c}{Gradient-free methods} \\
%         \midrule
%         LP & 76.0 (2.8)	& 40.3 (1.9) & 66.0 (2.7) & 56.5 (2.5) & 59.4 (5.3)	& 51.3 (5.5)\\
%         ZO \\
%         % ZO-Adam \\
%         % LP-ZO-SGD \\
%         ZO-LoRA \\
%         ZO-Prefix \\
%         
%         \midrule
%         
%         \bottomrule
%         \end{tabular}}
%         \caption{
%         Experiments on RoBERTa-large    
%         }
%         \label{tab:summary}
%     \end{table*}

==> tables/quant.tex <==
% \captionsetup[wrapfigure]{name=Table}

% \begin{wrapfigure}{r}{0.4\textwidth}
% \begin{minipage}{0.4\textwidth}

\begin{table}[h]
\small
\centering
%\resizebox{0.99\textwidth}{!}{
    \begin{tabular}{lcc}
    \toprule
     Task  & \tf{SST-2} & \tf{SQuAD} \\
    % Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
    \midrule
    % \midrule
    FP32 &  \\
    FP16 &  \\
    BF16 &  \\
    INT8 &  \\
    \bottomrule
    \end{tabular}%}
    \caption{
        Training with low-precision models.
    }
    \label{tab:quant}
\end{table}
% \end{minipage}
% \end{wrapfigure}


% \begin{table*}[t]
%     \centering
%     \small
%         \begin{tabular}{lcccccc}
%         \toprule
%          Task  &  \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{TREC}} \\
%         Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
%         % eNTK solves task & \checkmark & \checkmark & \checkmark & \checkmark & (\checkmark) & \checkmark & & \checkmark & & & (\checkmark) & \checkmark & \checkmark & \checkmark\\
%         % Linearization & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & \checkmark & \checkmark & \checkmark & \checkmark  \\
%         % Fixed Features & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
%         % \midrule
%         % Kernel behavior & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & (\checkmark) & \checkmark & \checkmark & \checkmark \\
%         \midrule
%         Zero-shot & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0 \\
%         \midrule
%         \multicolumn{7}{c}{Gradient-based methods: $16$-shot} \\
%         \midrule
%         Adam FT \\
%         SGD FT \\
%         LP-FT \\
%         LoRA FT \\
%         Prefix FT \\
%         \midrule
%         \multicolumn{7}{c}{Gradient-free methods: $16$-shot} \\
%         \midrule
%         LP \\
%         ZO-SGD \\
%         ZO-Adam \\
%         LP-ZO-SGD \\
%         ZO-LoRA \\
%         ZO-Prefix \\
%         
%         \midrule
%         
%         \bottomrule
%         \end{tabular}
%         \caption{
%         Experiments on RoBERTa-large    
%         }
%         \label{tab:summary}
%     \end{table*}

% \begin{table*}[t]
%     \centering
%     \resizebox{0.98\linewidth}{!}{
%         \begin{tabular}{lcccccc|cccccc}
%         \toprule
%         & \multicolumn{6}{c}{\textbf{$16$ examples per class}} & \multicolumn{6}{c}{\textbf{$512$ examples per class}}\\
%         \cmidrule(lr){2-7}\cmidrule(lr){8-13}
%          Task  &  \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c|}{\textbf{TREC}} & \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{SST-5}} & \multicolumn{1}{c}{\textbf{SNLI}}  & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{RTE}} & \multicolumn{1}{c}{\textbf{TREC}} \\
%         Task type & \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c|}{-- topic clf. --}& \multicolumn{2}{c}{---- sentiment ----} & \multicolumn{3}{c}{------ entailment ------} & \multicolumn{1}{c}{-- topic clf. --}\\
%         % eNTK solves task & \checkmark & \checkmark & \checkmark & \checkmark & (\checkmark) & \checkmark & & \checkmark & & & (\checkmark) & \checkmark & \checkmark & \checkmark\\
%         % Linearization & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & \checkmark & \checkmark & \checkmark & \checkmark  \\
%         % Fixed Features & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
%         % \midrule
%         % Kernel behavior & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & (\checkmark) & \checkmark & \checkmark & \checkmark \\
%         %\midrule
%         Zero-shot & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0 & 79.0 & 35.5 & 50.2 & 48.8 & 51.4 & 32.0\\
%         \midrule
%         \multicolumn{13}{c}{Gradient-based methods} \\
%         \midrule
%         FT \\
%         % SGD FT \\
%         % LP-FT \\
%         LoRA FT \\
%         Prefix FT \\
%         \midrule
%         \multicolumn{13}{c}{Gradient-free methods} \\
%         \midrule
%         LP & 76.0 (2.8)	& 40.3 (1.9) & 66.0 (2.7) & 56.5 (2.5) & 59.4 (5.3)	& 51.3 (5.5)\\
%         ZO \\
%         % ZO-Adam \\
%         % LP-ZO-SGD \\
%         ZO-LoRA \\
%         ZO-Prefix \\
%         
%         \midrule
%         
%         \bottomrule
%         \end{tabular}}
%         \caption{
%         Experiments on RoBERTa-large    
%         }
%         \label{tab:summary}
%     \end{table*}

==> tables/spsa_vs_zeroshot.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
         & SST-2  & SNLI & MRPC & TREC & BB-1 & BB-2 & BB-3 & BB-4 \\ \hline
         Zero-Shot & & & \\
         ZO-SGD ($K=16$) & & & \\
         ZO-Adam ($K=16$) & & & \\
         ZO-SGD (full-shot) & & & \\
         ZO-Adam (full-shot) & & & 
    \end{tabular}
    
    \caption{Comparing zero shot performance to few-shot and full-shot ZO-SGD and ZO-Adam for RoBERTa-large and OPT-175B on various GLUE and BigBench (BB) tasks. Turn this into a fancy table with RoBERTa-large as a header over GLUE tasks and OPT-175B over BB tasks.}
    \label{tab:spsa_works}
\end{table}

==> tables/workshop_zo_alg.tex <==
\vspace{-10pt}
\begin{algorithm}
  \SetKwFunction{perturb}{PerturbParameters}
  \SetKwProg{sub}{Subroutine}{}{}
  \SetKwComment{Comment}{$\triangleright$\ }{}
  
  %\KwIn{Initial parameter $\theta$, perturbation size $\epsilon$, and number of iterations $L$}
  %\KwOut{Optimal parameter $\theta^*$}
  \textbf{Require}: parameters $\vtheta\in\RR^d$, 
  loss $\cL:\RR^d\to\RR$, 
  step budget $T$,
  % loss $\cL\in \RR$, 
  perturbation scale $\epsilon$, 
  batch size $B$,
  learning rate schedule $\{\eta_t\}$ \\
  % \tnote{here loss is not necessarily $\RR^d\to \RR$?} \\
  \For{$t=1,...,T$} { %\danqi{$t = 1, \ldots, T$?}
    Sample batch $\cB\subset \cD$ and random seed $s$ \\
    %\danqi{Why do you need a random seed every time?} \\
    $\vtheta\gets$ \perturb{$\vtheta, \epsilon, s$} \\
    $\ell_+\gets\cL(\vtheta;\cB)$ \\
    $\vtheta\gets$ \perturb{$\vtheta, -2\epsilon, s$} \\
    $\ell_-\gets\cL(\vtheta;\cB)$ \\
    $\vtheta\gets$ \perturb{$\vtheta, \epsilon, s$} 
    \BlankLine
    $\texttt{projected\_grad}\gets (\ell_+ - \ell_-) / (2\epsilon)$ \\
    Reset random number generator with seed $s$ \\% \\ % \danqi{You don't need this line anymore, as long as $s$ is combined with sampling $z$.} \\ 
    \For{$\theta_i\in\vtheta$}{
        $z\sim\cN(0,1)$ \\
        %\danqi{I didn't see you reset the random seed earlier. I think you should just put $s$ in $\cN(\cdot)$} \\ 
        $\theta_i\gets\theta_i - \eta_t * \texttt{projected\_grad} * z$  
        %\Comment*[f]{\todo{Technically this can also be a call to perturb parameters, but not sure if it hurts clarity} \tnote{i think this is fine}}
    }
  }
  \sub{\perturb{$\vtheta$, $\epsilon$, $s$}}{
  Reset random number generator with seed $s$ \\
  %\Comment*[h]{$\theta_i$ is a parameter group that can be set at any scale. Setting a larger parameter group will increase the memory overhead but reduce the time.}\\
    \For{$\theta_i\in\vtheta$ }{  
      %\hskip\algorithmicindent \Comment*[r]{$\theta_i$ is a parameter group} 
        $z\sim\cN(0,1)$ \\
        $\theta_i\gets\theta_i+\epsilon z$ 
    }
    \Return $\vtheta$
  }
  
  \caption{\mezo{}}
  

  \label{alg:zo_sgd}
\end{algorithm}
\vspace{-15pt}

==> zo-ft-large.tex <==
\def\usebigfont{1}
\input{main}
